ALMol: Aligned Language-Molecule Translation LLMs through Offline Preference Contrastive Optimisation

The field of chemistry and Artificial Intelligence (AI) intersection is an area of active research that aims to accelerate scientific discovery. The integration of large language models (LLMs) with scientific modalities has shown significant promise in this endeavour. However, challenges persist in effectively addressing training efficacy and the out-of-distribution problem, particularly as existing approaches rely on larger models and datasets. In this context, we focus on machine language-molecule translation and deploy a novel training approach called contrastive preference optimisation, which avoids generating translations that are merely adequate but not perfect. To ensure generalisability and mitigate memorisation effects, we conduct experiments using only 10% of the data. Our results demonstrate that our models achieve up to a 32% improvement compared to counterpart models. Finally, we introduce a fine-grained, domain-agnostic evaluation method to assess hallucination in LLMs and promote responsible use.

==> task.tex <==
\section{Task Formulation}

Let $L$ denote the source language space and $M$ denote the target molecule space. Consider a dataset $\mathcal{D}$, comprising pairs of source language sequences $x$ represented in space $L$, and their corresponding target molecule sequences $y$ in space $M$, represented as $\mathcal{D}=\{x^{(i)},y^{(i)}\}_{i=1}^N$, where $N$ is the total number of pairs. Here, we cast the problem on a machine translation task, aiming to learn an optimal function $f: L \leftrightarrow M$ through a model $\pi_{\theta}$ parameterised by $\theta$. The dataset $\mathcal{D}$ comprises instructions, attaching task-specific prefixes at the beginning of $x$, which direct the translation direction, i.e., either $L \rightarrow M$ or $M \rightarrow L$.
